Preserve Your Own Correlation: A Noise Prior for Video Diffusion Models

Despite tremendous progress in generating high-quality images using diffusion models, synthesizing a sequence of animated frames that are both photorealistic and temporally coherent is still in its infancy. While off-the-shelf billion-scale datasets for image generation are available, collecting similar video data of the same scale is still challenging. Also, training a video diffusion model is computationally much more expensive than its image counterpart. In this work, we explore finetuning a pretrained image diffusion model with video data as a practical solution for the video synthesis task. We find that naively extending the image noise prior to video noise prior in video diffusion leads to sub-optimal performance. Our carefully designed video noise prior leads to substantially better performance. Extensive experimental validation shows that our model, Preserve Your Own Correlation (PYoCo), attains SOTA zero-shot text-to-video results on the UCF-101 and MSR-VTT benchmarks. It also achieves SOTA video generation quality on the small-scale UCF-101 benchmark with a $10\times$ smaller model using significantly less computation than the prior art.

==> figures/hyperparameter_for_ours.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth, trim=90 0 90 15, clip]{figures/alpha_sweep/alpha_sweep_FVD.png}
    \includegraphics[width=\linewidth, trim=90 0 90 15, clip]{figures/alpha_sweep/alpha_sweep_IS.png}
    \caption{\textbf{Ablation on the hyperparameter $\alpha$.} Finetuning with temporally correlated prior improves over training from scratch. Too large or too small $\alpha$s lead to inferior results. $\alpha=1$ works the best for mixed kaal and $\alpha=2$ works the best for progressive kaal.}
    \label{fig:sweep_alpha}
\end{figure}

==> figures/model_efficiency.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth, trim=90 0 90 15, clip]{figures/modelsize_sweep.png}
    \caption{\textbf{Ablation on model sizes.} Larger models consistently improve the performance of both finetuning and training from scratch. Finetuning consistently outperforms training from scratch.}
    \label{fig:sweep_modelsize}
\end{figure}

==> setup/graphicspath.tex <==
\graphicspath{{figures}, {examples}}


==> setup/package.tex <==
% % Fix "undefined control sequence \Everyshipout".
% % \usepackage{everyshi}

% % Figures
% \usepackage{graphicx}
% \usepackage{subcaption}
% \usepackage{float}
% \usepackage[justification=raggedright]{caption}	% makes captions ragged right - thanks to Bryce Lobdell
% \usepackage{lscape}                                         % Useful for wide tables or figures.
% \usepackage{wrapfig}

% % Algorithm
% \usepackage[lined,ruled,linesnumbered]{algorithm2e}
% \usepackage{animate} %% convert frames to video

% % Table and list
% \usepackage{booktabs}                   % Publication quality tables
% \usepackage{multirow}

% \usepackage{makecell}

% \usepackage{paralist}
% \usepackage{enumitem}
% \setlist[enumerate]{itemsep=0mm}

% % Math
% \usepackage{bm}                          % Make bold, italic math symbols
% \usepackage{epsfig}                      % for figures
% \usepackage{graphicx}                  % another package that works for figures
% \usepackage{times}
% \usepackage{mathptmx}
% \usepackage{mathtools}
% \usepackage{amssymb,amsmath}   % Short math guide for LaTeX ftp://ftp.ams.org/pub/tex/doc/amsmath/short-math-guide.pdf

% % Fonts
\usepackage{units}
\usepackage{color}

% % Comments
% \usepackage{comment}

% % Hyperlinks
% \usepackage{url}  % Hyphenation of URLs.
% %\usepackage[pagebackref=true,breaklinks=true,letterpaper=true,pagebackref=true,colorlinks,bookmarks=false]{hyperref}
% \usepackage[pagebackref,breaklinks,colorlinks,linkcolor=blue,citecolor=blue,urlcolor=blue,bookmarks=false]{hyperref}
% % \usepackage{authblk}
% % \usepackage{slashbox}
% \usepackage{xspace}
% \usepackage[table]{xcolor}
% \usepackage{setspace}
% \usepackage{grfext}
% \PrependGraphicsExtensions*{.jpg,.png,.PNG}

% \usepackage{gensymb}
% % \usepackage{emoji}

